HALS: A Height-Aware Lidar Super-Resolution Framework for Autonomous Driving

Lidar sensors are costly yet critical for understanding the 3D environment in autonomous driving. High-resolution sensors provide more details about the surroundings because they contain more vertical beams, but they come at a much higher cost, limiting their inclusion in autonomous vehicles. Upsampling lidar pointclouds is a promising approach to gain the benefits of high resolution while maintaining an affordable cost. Although there exist many pointcloud upsampling frameworks, a consistent comparison of these works against each other on the same dataset using unified metrics is still missing. In the first part of this paper, we propose to benchmark existing methods on the Kitti dataset. In the second part, we introduce a novel lidar upsampling model, HALS: Height-Aware Lidar Super-resolution. HALS exploits the observation that lidar scans exhibit a height-aware range distribution and adopts a generator architecture with multiple upsampling branches of different receptive fields. HALS regresses polar coordinates instead of spherical coordinates and uses a surface-normal loss. Extensive experiments show that HALS achieves state-of-the-art performance on 3 real-world lidar datasets.

==> Figures/DRB.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/DRB_block.pdf}
    \caption{Architecture of Dilated Resiudal Block (DRB)}
    \label{fig:drb}
    \vspace{-1em}
\end{figure}

==> Figures/Kitti_Object_Dataset.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=2.4in,
height=1.875in,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Beam ID},
xmin=-3.34, xmax=66.84,
xtick style={color=black},
y grid style={darkgray176},
ylabel=\textcolor{black}{Normalized Range},
ymin=0, ymax=0.336,
ytick style={color=black}
]
\draw[draw=none,fill=red] (axis cs:-0.15,0) rectangle (axis cs:0.15,0.31);
\draw[draw=none,fill=red] (axis cs:0.85,0) rectangle (axis cs:1.15,0.31);
\draw[draw=none,fill=red] (axis cs:1.85,0) rectangle (axis cs:2.15,0.32);
\draw[draw=none,fill=red] (axis cs:2.85,0) rectangle (axis cs:3.15,0.31);
\draw[draw=none,fill=red] (axis cs:3.85,0) rectangle (axis cs:4.15,0.31);
\draw[draw=none,fill=red] (axis cs:4.85,0) rectangle (axis cs:5.15,0.31);
\draw[draw=none,fill=red] (axis cs:5.85,0) rectangle (axis cs:6.15,0.3);
\draw[draw=none,fill=red] (axis cs:6.85,0) rectangle (axis cs:7.15,0.29);
\draw[draw=none,fill=red] (axis cs:7.85,0) rectangle (axis cs:8.15,0.28);
\draw[draw=none,fill=red] (axis cs:8.85,0) rectangle (axis cs:9.15,0.27);
\draw[draw=none,fill=red] (axis cs:9.85,0) rectangle (axis cs:10.15,0.25);
\draw[draw=none,fill=red] (axis cs:10.85,0) rectangle (axis cs:11.15,0.24);
\draw[draw=none,fill=red] (axis cs:11.85,0) rectangle (axis cs:12.15,0.23);
\draw[draw=none,fill=red] (axis cs:12.85,0) rectangle (axis cs:13.15,0.22);
\draw[draw=none,fill=red] (axis cs:13.85,0) rectangle (axis cs:14.15,0.2);
\draw[draw=none,fill=red] (axis cs:14.85,0) rectangle (axis cs:15.15,0.19);
\draw[draw=none,fill=red] (axis cs:15.85,0) rectangle (axis cs:16.15,0.18);
\draw[draw=none,fill=red] (axis cs:16.85,0) rectangle (axis cs:17.15,0.17);
\draw[draw=none,fill=red] (axis cs:17.85,0) rectangle (axis cs:18.15,0.17);
\draw[draw=none,fill=red] (axis cs:18.85,0) rectangle (axis cs:19.15,0.16);
\draw[draw=none,fill=red] (axis cs:19.85,0) rectangle (axis cs:20.15,0.15);
\draw[draw=none,fill=red] (axis cs:20.85,0) rectangle (axis cs:21.15,0.15);
\draw[draw=none,fill=red] (axis cs:21.85,0) rectangle (axis cs:22.15,0.14);
\draw[draw=none,fill=red] (axis cs:22.85,0) rectangle (axis cs:23.15,0.14);
\draw[draw=none,fill=red] (axis cs:23.85,0) rectangle (axis cs:24.15,0.12);
\draw[draw=none,fill=red] (axis cs:24.85,0) rectangle (axis cs:25.15,0.11);
\draw[draw=none,fill=red] (axis cs:25.85,0) rectangle (axis cs:26.15,0.12);
\draw[draw=none,fill=red] (axis cs:26.85,0) rectangle (axis cs:27.15,0.11);
\draw[draw=none,fill=red] (axis cs:27.85,0) rectangle (axis cs:28.15,0.11);
\draw[draw=none,fill=red] (axis cs:28.85,0) rectangle (axis cs:29.15,0.11);
\draw[draw=none,fill=red] (axis cs:29.85,0) rectangle (axis cs:30.15,0.1);
\draw[draw=none,fill=red] (axis cs:30.85,0) rectangle (axis cs:31.15,0.1);
\draw[draw=none,fill=red] (axis cs:31.85,0) rectangle (axis cs:32.15,0.1);
\draw[draw=none,fill=red] (axis cs:32.85,0) rectangle (axis cs:33.15,0.09);
\draw[draw=none,fill=red] (axis cs:33.85,0) rectangle (axis cs:34.15,0.09);
\draw[draw=none,fill=red] (axis cs:34.85,0) rectangle (axis cs:35.15,0.08);
\draw[draw=none,fill=red] (axis cs:35.85,0) rectangle (axis cs:36.15,0.09);
\draw[draw=none,fill=red] (axis cs:36.85,0) rectangle (axis cs:37.15,0.09);
\draw[draw=none,fill=red] (axis cs:37.85,0) rectangle (axis cs:38.15,0.08);
\draw[draw=none,fill=red] (axis cs:38.85,0) rectangle (axis cs:39.15,0.08);
\draw[draw=none,fill=red] (axis cs:39.85,0) rectangle (axis cs:40.15,0.08);
\draw[draw=none,fill=red] (axis cs:40.85,0) rectangle (axis cs:41.15,0.08);
\draw[draw=none,fill=red] (axis cs:41.85,0) rectangle (axis cs:42.15,0.07);
\draw[draw=none,fill=red] (axis cs:42.85,0) rectangle (axis cs:43.15,0.07);
\draw[draw=none,fill=red] (axis cs:43.85,0) rectangle (axis cs:44.15,0.07);
\draw[draw=none,fill=red] (axis cs:44.85,0) rectangle (axis cs:45.15,0.07);
\draw[draw=none,fill=red] (axis cs:45.85,0) rectangle (axis cs:46.15,0.07);
\draw[draw=none,fill=red] (axis cs:46.85,0) rectangle (axis cs:47.15,0.07);
\draw[draw=none,fill=red] (axis cs:47.85,0) rectangle (axis cs:48.15,0.07);
\draw[draw=none,fill=red] (axis cs:48.85,0) rectangle (axis cs:49.15,0.06);
\draw[draw=none,fill=red] (axis cs:49.85,0) rectangle (axis cs:50.15,0.06);
\draw[draw=none,fill=red] (axis cs:50.85,0) rectangle (axis cs:51.15,0.06);
\draw[draw=none,fill=red] (axis cs:51.85,0) rectangle (axis cs:52.15,0.06);
\draw[draw=none,fill=red] (axis cs:52.85,0) rectangle (axis cs:53.15,0.06);
\draw[draw=none,fill=red] (axis cs:53.85,0) rectangle (axis cs:54.15,0.06);
\draw[draw=none,fill=red] (axis cs:54.85,0) rectangle (axis cs:55.15,0.06);
\draw[draw=none,fill=red] (axis cs:55.85,0) rectangle (axis cs:56.15,0.06);
\draw[draw=none,fill=red] (axis cs:56.85,0) rectangle (axis cs:57.15,0.06);
\draw[draw=none,fill=red] (axis cs:57.85,0) rectangle (axis cs:58.15,0.06);
\draw[draw=none,fill=red] (axis cs:58.85,0) rectangle (axis cs:59.15,0.05);
\draw[draw=none,fill=red] (axis cs:59.85,0) rectangle (axis cs:60.15,0.05);
\draw[draw=none,fill=red] (axis cs:60.85,0) rectangle (axis cs:61.15,0.06);
\draw[draw=none,fill=red] (axis cs:61.85,0) rectangle (axis cs:62.15,0.03);
\draw[draw=none,fill=red] (axis cs:62.85,0) rectangle (axis cs:63.15,0.03);
\draw[draw=none,fill=blue] (axis cs:0.35,0) rectangle (axis cs:0.65,0.19);
\draw[draw=none,fill=blue] (axis cs:1.35,0) rectangle (axis cs:1.65,0.19);
\draw[draw=none,fill=blue] (axis cs:2.35,0) rectangle (axis cs:2.65,0.2);
\draw[draw=none,fill=blue] (axis cs:3.35,0) rectangle (axis cs:3.65,0.2);
\draw[draw=none,fill=blue] (axis cs:4.35,0) rectangle (axis cs:4.65,0.19);
\draw[draw=none,fill=blue] (axis cs:5.35,0) rectangle (axis cs:5.65,0.19);
\draw[draw=none,fill=blue] (axis cs:6.35,0) rectangle (axis cs:6.65,0.19);
\draw[draw=none,fill=blue] (axis cs:7.35,0) rectangle (axis cs:7.65,0.18);
\draw[draw=none,fill=blue] (axis cs:8.35,0) rectangle (axis cs:8.65,0.17);
\draw[draw=none,fill=blue] (axis cs:9.35,0) rectangle (axis cs:9.65,0.16);
\draw[draw=none,fill=blue] (axis cs:10.35,0) rectangle (axis cs:10.65,0.14);
\draw[draw=none,fill=blue] (axis cs:11.35,0) rectangle (axis cs:11.65,0.13);
\draw[draw=none,fill=blue] (axis cs:12.35,0) rectangle (axis cs:12.65,0.12);
\draw[draw=none,fill=blue] (axis cs:13.35,0) rectangle (axis cs:13.65,0.1);
\draw[draw=none,fill=blue] (axis cs:14.35,0) rectangle (axis cs:14.65,0.09);
\draw[draw=none,fill=blue] (axis cs:15.35,0) rectangle (axis cs:15.65,0.08);
\draw[draw=none,fill=blue] (axis cs:16.35,0) rectangle (axis cs:16.65,0.07);
\draw[draw=none,fill=blue] (axis cs:17.35,0) rectangle (axis cs:17.65,0.06);
\draw[draw=none,fill=blue] (axis cs:18.35,0) rectangle (axis cs:18.65,0.06);
\draw[draw=none,fill=blue] (axis cs:19.35,0) rectangle (axis cs:19.65,0.05);
\draw[draw=none,fill=blue] (axis cs:20.35,0) rectangle (axis cs:20.65,0.05);
\draw[draw=none,fill=blue] (axis cs:21.35,0) rectangle (axis cs:21.65,0.04);
\draw[draw=none,fill=blue] (axis cs:22.35,0) rectangle (axis cs:22.65,0.04);
\draw[draw=none,fill=blue] (axis cs:23.35,0) rectangle (axis cs:23.65,0.04);
\draw[draw=none,fill=blue] (axis cs:24.35,0) rectangle (axis cs:24.65,0.03);
\draw[draw=none,fill=blue] (axis cs:25.35,0) rectangle (axis cs:25.65,0.03);
\draw[draw=none,fill=blue] (axis cs:26.35,0) rectangle (axis cs:26.65,0.03);
\draw[draw=none,fill=blue] (axis cs:27.35,0) rectangle (axis cs:27.65,0.02);
\draw[draw=none,fill=blue] (axis cs:28.35,0) rectangle (axis cs:28.65,0.02);
\draw[draw=none,fill=blue] (axis cs:29.35,0) rectangle (axis cs:29.65,0.02);
\draw[draw=none,fill=blue] (axis cs:30.35,0) rectangle (axis cs:30.65,0.02);
\draw[draw=none,fill=blue] (axis cs:31.35,0) rectangle (axis cs:31.65,0.02);
\draw[draw=none,fill=blue] (axis cs:32.35,0) rectangle (axis cs:32.65,0.02);
\draw[draw=none,fill=blue] (axis cs:33.35,0) rectangle (axis cs:33.65,0.02);
\draw[draw=none,fill=blue] (axis cs:34.35,0) rectangle (axis cs:34.65,0.01);
\draw[draw=none,fill=blue] (axis cs:35.35,0) rectangle (axis cs:35.65,0.01);
\draw[draw=none,fill=blue] (axis cs:36.35,0) rectangle (axis cs:36.65,0.01);
\draw[draw=none,fill=blue] (axis cs:37.35,0) rectangle (axis cs:37.65,0.01);
\draw[draw=none,fill=blue] (axis cs:38.35,0) rectangle (axis cs:38.65,0.01);
\draw[draw=none,fill=blue] (axis cs:39.35,0) rectangle (axis cs:39.65,0.01);
\draw[draw=none,fill=blue] (axis cs:40.35,0) rectangle (axis cs:40.65,0.01);
\draw[draw=none,fill=blue] (axis cs:41.35,0) rectangle (axis cs:41.65,0.01);
\draw[draw=none,fill=blue] (axis cs:42.35,0) rectangle (axis cs:42.65,0.01);
\draw[draw=none,fill=blue] (axis cs:43.35,0) rectangle (axis cs:43.65,0.01);
\draw[draw=none,fill=blue] (axis cs:44.35,0) rectangle (axis cs:44.65,0.01);
\draw[draw=none,fill=blue] (axis cs:45.35,0) rectangle (axis cs:45.65,0.01);
\draw[draw=none,fill=blue] (axis cs:46.35,0) rectangle (axis cs:46.65,0.01);
\draw[draw=none,fill=blue] (axis cs:47.35,0) rectangle (axis cs:47.65,0.01);
\draw[draw=none,fill=blue] (axis cs:48.35,0) rectangle (axis cs:48.65,0.01);
\draw[draw=none,fill=blue] (axis cs:49.35,0) rectangle (axis cs:49.65,0.01);
\draw[draw=none,fill=blue] (axis cs:50.35,0) rectangle (axis cs:50.65,0.01);
\draw[draw=none,fill=blue] (axis cs:51.35,0) rectangle (axis cs:51.65,0.01);
\draw[draw=none,fill=blue] (axis cs:52.35,0) rectangle (axis cs:52.65,0.01);
\draw[draw=none,fill=blue] (axis cs:53.35,0) rectangle (axis cs:53.65,0.01);
\draw[draw=none,fill=blue] (axis cs:54.35,0) rectangle (axis cs:54.65,0.01);
\draw[draw=none,fill=blue] (axis cs:55.35,0) rectangle (axis cs:55.65,0.01);
\draw[draw=none,fill=blue] (axis cs:56.35,0) rectangle (axis cs:56.65,0.01);
\draw[draw=none,fill=blue] (axis cs:57.35,0) rectangle (axis cs:57.65,0.02);
\draw[draw=none,fill=blue] (axis cs:58.35,0) rectangle (axis cs:58.65,0.01);
\draw[draw=none,fill=blue] (axis cs:59.35,0) rectangle (axis cs:59.65,0.01);
\draw[draw=none,fill=blue] (axis cs:60.35,0) rectangle (axis cs:60.65,0);
\draw[draw=none,fill=blue] (axis cs:61.35,0) rectangle (axis cs:61.65,0.01);
\draw[draw=none,fill=blue] (axis cs:62.35,0) rectangle (axis cs:62.65,0);
\draw[draw=none,fill=blue] (axis cs:63.35,0) rectangle (axis cs:63.65,0);
\end{axis}


\end{tikzpicture}


==> Figures/Kitti_Raw_Dataset.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=2.4in,
height=1.875in,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Beam ID},
xmin=-2.14, xmax=41.64,
xtick style={color=black},
y grid style={darkgray176},
ylabel=\textcolor{black}{Normalized Range},
ymin=0, ymax=0.3045,
ytick style={color=black}
]
\draw[draw=none,fill=red] (axis cs:-0.15,0) rectangle (axis cs:0.15,0.29);
\draw[draw=none,fill=red] (axis cs:0.85,0) rectangle (axis cs:1.15,0.28);
\draw[draw=none,fill=red] (axis cs:1.85,0) rectangle (axis cs:2.15,0.27);
\draw[draw=none,fill=red] (axis cs:2.85,0) rectangle (axis cs:3.15,0.26);
\draw[draw=none,fill=red] (axis cs:3.85,0) rectangle (axis cs:4.15,0.25);
\draw[draw=none,fill=red] (axis cs:4.85,0) rectangle (axis cs:5.15,0.24);
\draw[draw=none,fill=red] (axis cs:5.85,0) rectangle (axis cs:6.15,0.23);
\draw[draw=none,fill=red] (axis cs:6.85,0) rectangle (axis cs:7.15,0.23);
\draw[draw=none,fill=red] (axis cs:7.85,0) rectangle (axis cs:8.15,0.22);
\draw[draw=none,fill=red] (axis cs:8.85,0) rectangle (axis cs:9.15,0.21);
\draw[draw=none,fill=red] (axis cs:9.85,0) rectangle (axis cs:10.15,0.2);
\draw[draw=none,fill=red] (axis cs:10.85,0) rectangle (axis cs:11.15,0.2);
\draw[draw=none,fill=red] (axis cs:11.85,0) rectangle (axis cs:12.15,0.19);
\draw[draw=none,fill=red] (axis cs:12.85,0) rectangle (axis cs:13.15,0.19);
\draw[draw=none,fill=red] (axis cs:13.85,0) rectangle (axis cs:14.15,0.18);
\draw[draw=none,fill=red] (axis cs:14.85,0) rectangle (axis cs:15.15,0.17);
\draw[draw=none,fill=red] (axis cs:15.85,0) rectangle (axis cs:16.15,0.16);
\draw[draw=none,fill=red] (axis cs:16.85,0) rectangle (axis cs:17.15,0.16);
\draw[draw=none,fill=red] (axis cs:17.85,0) rectangle (axis cs:18.15,0.15);
\draw[draw=none,fill=red] (axis cs:18.85,0) rectangle (axis cs:19.15,0.15);
\draw[draw=none,fill=red] (axis cs:19.85,0) rectangle (axis cs:20.15,0.14);
\draw[draw=none,fill=red] (axis cs:20.85,0) rectangle (axis cs:21.15,0.14);
\draw[draw=none,fill=red] (axis cs:21.85,0) rectangle (axis cs:22.15,0.13);
\draw[draw=none,fill=red] (axis cs:22.85,0) rectangle (axis cs:23.15,0.13);
\draw[draw=none,fill=red] (axis cs:23.85,0) rectangle (axis cs:24.15,0.12);
\draw[draw=none,fill=red] (axis cs:24.85,0) rectangle (axis cs:25.15,0.12);
\draw[draw=none,fill=red] (axis cs:25.85,0) rectangle (axis cs:26.15,0.12);
\draw[draw=none,fill=red] (axis cs:26.85,0) rectangle (axis cs:27.15,0.11);
\draw[draw=none,fill=red] (axis cs:27.85,0) rectangle (axis cs:28.15,0.11);
\draw[draw=none,fill=red] (axis cs:28.85,0) rectangle (axis cs:29.15,0.1);
\draw[draw=none,fill=red] (axis cs:29.85,0) rectangle (axis cs:30.15,0.1);
\draw[draw=none,fill=red] (axis cs:30.85,0) rectangle (axis cs:31.15,0.1);
\draw[draw=none,fill=red] (axis cs:31.85,0) rectangle (axis cs:32.15,0.1);
\draw[draw=none,fill=red] (axis cs:32.85,0) rectangle (axis cs:33.15,0.09);
\draw[draw=none,fill=red] (axis cs:33.85,0) rectangle (axis cs:34.15,0.09);
\draw[draw=none,fill=red] (axis cs:34.85,0) rectangle (axis cs:35.15,0.09);
\draw[draw=none,fill=red] (axis cs:35.85,0) rectangle (axis cs:36.15,0.09);
\draw[draw=none,fill=red] (axis cs:36.85,0) rectangle (axis cs:37.15,0.09);
\draw[draw=none,fill=red] (axis cs:37.85,0) rectangle (axis cs:38.15,0.09);
\draw[draw=none,fill=red] (axis cs:38.85,0) rectangle (axis cs:39.15,0.08);
\draw[draw=none,fill=blue] (axis cs:0.35,0) rectangle (axis cs:0.65,0.13);
\draw[draw=none,fill=blue] (axis cs:1.35,0) rectangle (axis cs:1.65,0.12);
\draw[draw=none,fill=blue] (axis cs:2.35,0) rectangle (axis cs:2.65,0.12);
\draw[draw=none,fill=blue] (axis cs:3.35,0) rectangle (axis cs:3.65,0.11);
\draw[draw=none,fill=blue] (axis cs:4.35,0) rectangle (axis cs:4.65,0.1);
\draw[draw=none,fill=blue] (axis cs:5.35,0) rectangle (axis cs:5.65,0.09);
\draw[draw=none,fill=blue] (axis cs:6.35,0) rectangle (axis cs:6.65,0.08);
\draw[draw=none,fill=blue] (axis cs:7.35,0) rectangle (axis cs:7.65,0.07);
\draw[draw=none,fill=blue] (axis cs:8.35,0) rectangle (axis cs:8.65,0.07);
\draw[draw=none,fill=blue] (axis cs:9.35,0) rectangle (axis cs:9.65,0.06);
\draw[draw=none,fill=blue] (axis cs:10.35,0) rectangle (axis cs:10.65,0.06);
\draw[draw=none,fill=blue] (axis cs:11.35,0) rectangle (axis cs:11.65,0.05);
\draw[draw=none,fill=blue] (axis cs:12.35,0) rectangle (axis cs:12.65,0.05);
\draw[draw=none,fill=blue] (axis cs:13.35,0) rectangle (axis cs:13.65,0.05);
\draw[draw=none,fill=blue] (axis cs:14.35,0) rectangle (axis cs:14.65,0.04);
\draw[draw=none,fill=blue] (axis cs:15.35,0) rectangle (axis cs:15.65,0.04);
\draw[draw=none,fill=blue] (axis cs:16.35,0) rectangle (axis cs:16.65,0.04);
\draw[draw=none,fill=blue] (axis cs:17.35,0) rectangle (axis cs:17.65,0.03);
\draw[draw=none,fill=blue] (axis cs:18.35,0) rectangle (axis cs:18.65,0.03);
\draw[draw=none,fill=blue] (axis cs:19.35,0) rectangle (axis cs:19.65,0.03);
\draw[draw=none,fill=blue] (axis cs:20.35,0) rectangle (axis cs:20.65,0.03);
\draw[draw=none,fill=blue] (axis cs:21.35,0) rectangle (axis cs:21.65,0.02);
\draw[draw=none,fill=blue] (axis cs:22.35,0) rectangle (axis cs:22.65,0.02);
\draw[draw=none,fill=blue] (axis cs:23.35,0) rectangle (axis cs:23.65,0.02);
\draw[draw=none,fill=blue] (axis cs:24.35,0) rectangle (axis cs:24.65,0.02);
\draw[draw=none,fill=blue] (axis cs:25.35,0) rectangle (axis cs:25.65,0.02);
\draw[draw=none,fill=blue] (axis cs:26.35,0) rectangle (axis cs:26.65,0.02);
\draw[draw=none,fill=blue] (axis cs:27.35,0) rectangle (axis cs:27.65,0.02);
\draw[draw=none,fill=blue] (axis cs:28.35,0) rectangle (axis cs:28.65,0.01);
\draw[draw=none,fill=blue] (axis cs:29.35,0) rectangle (axis cs:29.65,0.01);
\draw[draw=none,fill=blue] (axis cs:30.35,0) rectangle (axis cs:30.65,0.01);
\draw[draw=none,fill=blue] (axis cs:31.35,0) rectangle (axis cs:31.65,0.01);
\draw[draw=none,fill=blue] (axis cs:32.35,0) rectangle (axis cs:32.65,0.01);
\draw[draw=none,fill=blue] (axis cs:33.35,0) rectangle (axis cs:33.65,0.01);
\draw[draw=none,fill=blue] (axis cs:34.35,0) rectangle (axis cs:34.65,0.01);
\draw[draw=none,fill=blue] (axis cs:35.35,0) rectangle (axis cs:35.65,0.01);
\draw[draw=none,fill=blue] (axis cs:36.35,0) rectangle (axis cs:36.65,0.01);
\draw[draw=none,fill=blue] (axis cs:37.35,0) rectangle (axis cs:37.65,0.01);
\draw[draw=none,fill=blue] (axis cs:38.35,0) rectangle (axis cs:38.65,0.01);
\draw[draw=none,fill=blue] (axis cs:39.35,0) rectangle (axis cs:39.65,0.01);
\end{axis}

\end{tikzpicture}


==> Figures/Nuscenes_Dataset.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
width=2.4in,
height=1.875in,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Beam ID},
xmin=-1.74, xmax=33.24,
xtick style={color=black},
y grid style={darkgray176},
ylabel=\textcolor{black}{Normalized Range},
ymin=0, ymax=0.294,
ytick style={color=black}
]
]
\draw[draw=none,fill=red] (axis cs:-0.15,0) rectangle (axis cs:0.15,0.26);
\draw[draw=none,fill=red] (axis cs:0.85,0) rectangle (axis cs:1.15,0.28);
\draw[draw=none,fill=red] (axis cs:1.85,0) rectangle (axis cs:2.15,0.28);
\draw[draw=none,fill=red] (axis cs:2.85,0) rectangle (axis cs:3.15,0.28);
\draw[draw=none,fill=red] (axis cs:3.85,0) rectangle (axis cs:4.15,0.28);
\draw[draw=none,fill=red] (axis cs:4.85,0) rectangle (axis cs:5.15,0.28);
\draw[draw=none,fill=red] (axis cs:5.85,0) rectangle (axis cs:6.15,0.28);
\draw[draw=none,fill=red] (axis cs:6.85,0) rectangle (axis cs:7.15,0.27);
\draw[draw=none,fill=red] (axis cs:7.85,0) rectangle (axis cs:8.15,0.25);
\draw[draw=none,fill=red] (axis cs:8.85,0) rectangle (axis cs:9.15,0.23);
\draw[draw=none,fill=red] (axis cs:9.85,0) rectangle (axis cs:10.15,0.21);
\draw[draw=none,fill=red] (axis cs:10.85,0) rectangle (axis cs:11.15,0.18);
\draw[draw=none,fill=red] (axis cs:11.85,0) rectangle (axis cs:12.15,0.15);
\draw[draw=none,fill=red] (axis cs:12.85,0) rectangle (axis cs:13.15,0.13);
\draw[draw=none,fill=red] (axis cs:13.85,0) rectangle (axis cs:14.15,0.11);
\draw[draw=none,fill=red] (axis cs:14.85,0) rectangle (axis cs:15.15,0.1);
\draw[draw=none,fill=red] (axis cs:15.85,0) rectangle (axis cs:16.15,0.09);
\draw[draw=none,fill=red] (axis cs:16.85,0) rectangle (axis cs:17.15,0.08);
\draw[draw=none,fill=red] (axis cs:17.85,0) rectangle (axis cs:18.15,0.08);
\draw[draw=none,fill=red] (axis cs:18.85,0) rectangle (axis cs:19.15,0.07);
\draw[draw=none,fill=red] (axis cs:19.85,0) rectangle (axis cs:20.15,0.06);
\draw[draw=none,fill=red] (axis cs:20.85,0) rectangle (axis cs:21.15,0.06);
\draw[draw=none,fill=red] (axis cs:21.85,0) rectangle (axis cs:22.15,0.06);
\draw[draw=none,fill=red] (axis cs:22.85,0) rectangle (axis cs:23.15,0.05);
\draw[draw=none,fill=red] (axis cs:23.85,0) rectangle (axis cs:24.15,0.05);
\draw[draw=none,fill=red] (axis cs:24.85,0) rectangle (axis cs:25.15,0.05);
\draw[draw=none,fill=red] (axis cs:25.85,0) rectangle (axis cs:26.15,0.04);
\draw[draw=none,fill=red] (axis cs:26.85,0) rectangle (axis cs:27.15,0.04);
\draw[draw=none,fill=red] (axis cs:27.85,0) rectangle (axis cs:28.15,0.04);
\draw[draw=none,fill=red] (axis cs:28.85,0) rectangle (axis cs:29.15,0.04);
\draw[draw=none,fill=red] (axis cs:29.85,0) rectangle (axis cs:30.15,0.04);
\draw[draw=none,fill=red] (axis cs:30.85,0) rectangle (axis cs:31.15,0.03);
\draw[draw=none,fill=blue] (axis cs:0.35,0) rectangle (axis cs:0.65,0.16);
\draw[draw=none,fill=blue] (axis cs:1.35,0) rectangle (axis cs:1.65,0.16);
\draw[draw=none,fill=blue] (axis cs:2.35,0) rectangle (axis cs:2.65,0.17);
\draw[draw=none,fill=blue] (axis cs:3.35,0) rectangle (axis cs:3.65,0.17);
\draw[draw=none,fill=blue] (axis cs:4.35,0) rectangle (axis cs:4.65,0.17);
\draw[draw=none,fill=blue] (axis cs:5.35,0) rectangle (axis cs:5.65,0.17);
\draw[draw=none,fill=blue] (axis cs:6.35,0) rectangle (axis cs:6.65,0.17);
\draw[draw=none,fill=blue] (axis cs:7.35,0) rectangle (axis cs:7.65,0.16);
\draw[draw=none,fill=blue] (axis cs:8.35,0) rectangle (axis cs:8.65,0.16);
\draw[draw=none,fill=blue] (axis cs:9.35,0) rectangle (axis cs:9.65,0.14);
\draw[draw=none,fill=blue] (axis cs:10.35,0) rectangle (axis cs:10.65,0.12);
\draw[draw=none,fill=blue] (axis cs:11.35,0) rectangle (axis cs:11.65,0.09);
\draw[draw=none,fill=blue] (axis cs:12.35,0) rectangle (axis cs:12.65,0.06);
\draw[draw=none,fill=blue] (axis cs:13.35,0) rectangle (axis cs:13.65,0.05);
\draw[draw=none,fill=blue] (axis cs:14.35,0) rectangle (axis cs:14.65,0.04);
\draw[draw=none,fill=blue] (axis cs:15.35,0) rectangle (axis cs:15.65,0.03);
\draw[draw=none,fill=blue] (axis cs:16.35,0) rectangle (axis cs:16.65,0.02);
\draw[draw=none,fill=blue] (axis cs:17.35,0) rectangle (axis cs:17.65,0.02);
\draw[draw=none,fill=blue] (axis cs:18.35,0) rectangle (axis cs:18.65,0.01);
\draw[draw=none,fill=blue] (axis cs:19.35,0) rectangle (axis cs:19.65,0.01);
\draw[draw=none,fill=blue] (axis cs:20.35,0) rectangle (axis cs:20.65,0.01);
\draw[draw=none,fill=blue] (axis cs:21.35,0) rectangle (axis cs:21.65,0.01);
\draw[draw=none,fill=blue] (axis cs:22.35,0) rectangle (axis cs:22.65,0.01);
\draw[draw=none,fill=blue] (axis cs:23.35,0) rectangle (axis cs:23.65,0.01);
\draw[draw=none,fill=blue] (axis cs:24.35,0) rectangle (axis cs:24.65,0.01);
\draw[draw=none,fill=blue] (axis cs:25.35,0) rectangle (axis cs:25.65,0.01);
\draw[draw=none,fill=blue] (axis cs:26.35,0) rectangle (axis cs:26.65,0.01);
\draw[draw=none,fill=blue] (axis cs:27.35,0) rectangle (axis cs:27.65,0.01);
\draw[draw=none,fill=blue] (axis cs:28.35,0) rectangle (axis cs:28.65,0.01);
\draw[draw=none,fill=blue] (axis cs:29.35,0) rectangle (axis cs:29.65,0.01);
\draw[draw=none,fill=blue] (axis cs:30.35,0) rectangle (axis cs:30.65,0.01);
\draw[draw=none,fill=blue] (axis cs:31.35,0) rectangle (axis cs:31.65,0.01);
\coordinate (legendPos) at (axis description cs:0.975,0.855);
\end{axis}

\node[anchor=east,text width=2.0cm,align=left,fill=white,draw=black!80,line width=0.1mm,font=\fontsize{10}{0}\selectfont] at (legendPos) {\ref{lab:patch} \small Mean \\ \vspace{1mm} \ref{lab:whole} \small Std};
\end{tikzpicture}


==> Tables/ablation.tex <==
\begin{table}[t]
\small
\centering 
\caption{Comparative and Ablation study on Kitti Benchmark, $\times4$ upsampling rate. The last row represents the complete proposed framework.}
\label{table:ablation}
\scalebox{0.9}{\begin{tabular}{l | c c c c} 
\Xhline{1pt}
Framework & \textbf{EMD} & \textbf{CD} & \textbf{MAE} & \textbf{RMSE} \\ 
\hline
SRResNet \cite{lidarsrresnet}      & 100.1 & 0.052 & 0.20 & 0.86 \\
UNet \cite{unetlidar}       & 101.0 & 0.054 & 0.21 & \textbf{0.85} \\
\hline
SRGAN \cite{srgan}        & 100.6 & 0.051 & 0.19 &  0.86 \\
  + VNL                   & 88.7 & 0.031 & 0.23 &  0.87  \\
  + VNL + cartesian       & 89.6 & 0.033 & 0.24 &  0.88  \\
  + VNL + polar           & 84.3 & 0.023 & 0.21 &  0.86 \\
  + DRB + VNL + polar (GLPU)     & \textbf{81.4} & \textbf{0.016} & \textbf{0.18} &  0.87 \\
\Xhline{1pt}
\end{tabular}}
\vspace{-1em}
\end{table}

==> draft.tex <==
%However,  because of the problem's complexity, it is unlikely that a single breakthrough would increase performance; instead, a combination of methods is needed. We identify four main challenges: 1) the input and output representation of lidar pointclouds, 2) the upsampling network's receptive field, 3) the loss function to lean high-frequencies, and 4) the handling of sparse locations in projected pointclouds. In short, the 4 problems stem from attempting to learn an upsampled pointcloud in an end-to-end manner with deep learning while neglecting the scene geometry. To circumvent these limitations, we propose the Geometric Lidar Pointcloud Upsampling (GLPU) framework that attends to the scene 3D geometry to overcome each of the mentioned limitations.


%although it had a lower performance than other point-based algorithms on the PUNet dataset. To identify the underlying reasons and gain more insights into the lidar upsampling task,


%We hypothesize that the standard use of MAE and MSE losses in these methods does not encourage the upsampling layer to produce high-frequencies in the range image, potentially leading to the loss of fine details in the scene.

%PUGAN~\cite{pugan}, a Pointnet-based network, was a pioneering work, although the downsampling and upsampling scheme used is different than this work (and the subsequently mentioned baselines). PUGAN first downsamples lidar pointclouds by dropping out points with a defined probability distribution. This scheme does not simulate lidar sensors of different vertical resolutions. In contrast, 

%HALS consists of two components: a 2D CNN generator $\mathcal{G}$, and a discriminator $\mathcal{D}$, trained in an adversarial manner. $\mathcal{G}$ takes a grid image $\mathcal{Q}_{LR}$ of the pointcloud $\mathcal{P}_{LR}$, where each pixel contains the polar coordinates $(d, z)$ of a point. $\mathcal{G}$ outputs a high-resolution range image in polar coordinates as well, $\hat{\mathcal{Q}}_{HR}$. On the other hand, $\mathcal{D}$ attempts to discriminate between real and generated range images in spherical coordinates. For this, we transform $\hat{\mathcal{Q}}_{HR}$ and the groundtruth $\mathcal{Q}_{HR}$ to spherical coordinates before passing them to the discriminator. All range images are normalized between $0$ and $1$ before training, by dividing the coordinates by the highest range value in the dataset. 

%\subsection{Dilated SR-ResNet}
%The second most important factor we have observed is the receptive field, which should capture local and global information in the pointcloud. The receptive field of the SRResNet in \cite{lidarsrresnet} is large enough in $H$ but not in $W$. On the other hand, the receptive field of the UNet in \cite{unetlidar} is large enough by virtue of the average pooling operations used but does not offer an advantage over SRResNet. Classes like pedestrians and cyclists which are very small compared to the whole lidar scene, might disappear after the average pooling. It is thus desirable to have a large receptive field without increasing the stride. Since naively increasing the kernel size will greatly increase the number of parameters in the network, we build our SRResNet-based generator architecture using the dilated residual blocks introduced in \cite{rangercnn} as can be see in in \cref{fig:method}. The dilated convolutions increase the size of the receptive field to detect objects of different scales without significantly increasing the number of parameters. The parallel design of the block also allows to flexibly capture coarse and fine details.
%\vspace{-1em}

%As previously noted, the choice of the pointcloud representation is crucial for the upsampling performance. The range image representation is a better fit for the task: first, 2D networks are not as computationally expensive as pointnet operations and second, it allows conv layers with small receptive fields to interpolate between vertical lines. However, the latter comes with a disadvantage: the distribution of distances exhibits a large variance in the vertical direction $H$ of the range image (the issue was also mentioned by \cite{semilocal}), impeding conv and upsampling layers from replicating these high-frequency components in the range image. The problem is further complicated by the use of spherical coordinates, whereby it is implicitly assumed that the elevation angle $\theta = arcsin(zr^{-1})$ is constant between all vertical lines. This assumption is not true and it introduces a quantization error when the inverse transformation from $\mathcal{Q}$ to $\mathcal{P}$ is applied, namely $z = rsin(\theta)$. 

%In order to force the upsampling layer (transposed conv layer) to produce more meaningful features, we penalize the deviation of the surface normal of the generated pointcloud from that of the groundtruth. However, instead of calculating the normal vector for every point in the range image, we use the virtual normal loss (VNL) proposed by \cite{vnl}.  


%We train all models for for $100$ epochs, with a batchsize of $32$ and ADAM optimizer with learning rate of $0.0001$. We perform and ablation study and report the results in \cref{table:ablation} and \cref{fig:results}. We also add the metrics MAE and RMSE to \cref{table:ablation}. MAE and RMSE are measured in meters, while CD is measured in $m^{2}$. Lower values indicate superior performance. 

%The results show that the proposed model outperforms the state-of-the-art models on the EMD, CD and MAE metrics and is on par on the RMSE metrics. However, we find that MAE and RMSE are not sufficient to judge the upsampling quality: the table shows that EMD and CD can differ significantly, while MAE and RMSE exhibit little variations. This observation is analogous to the findings in \cite{srgan}, where MAE and RMSE were found to be weakly correlated to RGB image quality. We also notice that the UNet model \cite{unetlidar} underperforms the basic SRResNet \cite{lidarsrresnet} on the proposed benchmark, contrary to the findings in \cite{unetlidar}. This difference can be attributed to the fact that synthetic lidar obtained from the CARLA simulator \cite{carla} was used for evaluation in \cite{unetlidar}, which is less noisier than real lidar data. 

%and that regressing ($d$, $z$) is sufficient to eliminate the quantization error in the vertical dimension

%In \cref{table:ablation}, an ablation study on our model showcases the contribution of each design choice. Although, the SRGAN itself does not improve the results significantly, when combined with the VNL, a clear reduction in EMD and CD can be seen. This shows that the proposed losses can guide the generator to produce a more coherent scene by enforcing a high-order constraint on the underlying scene geometry. The use of polar coordinates is shown to further improve the results, since it removes the vertical quantization error. On the other hand, cartesian coordinates do not show an improvement arguably because regressing $3$ channels is a more challenging task for the network. Finally, we find that the DRBs further enhance the performance, confirming our claim that the receptive field is a crucial design parameter for the task. 
%\vspace{-1em}

%Third, the downsampling and upsampling schemes of these algorithms are different. For example, methods based on Pointnet operators \cite{pointnet, punet, pugan, patchupsample, argcn} sample patches from the pointclouds with farthest sampling, downsample each patch and train their corresponding networks on upsampling the low-resolution patches. In contrast, \cite{deepgm} removes points from lidar scan with a uniform probability distribution and the whole pointcloud is reconstructed directly with a VAE \cite{vae}. A third scheme is presented in \cite{lidarsrresnet, unetlidar}, whereby lidar scans are downsampled in the vertical resolution by skipping every second beam and a 2D convolutional network attempts to upsample the pointcloud. To summarize, there has not been a consistent comparison of these frameworks on real scans. 

%After evaluating the existing works, we seek to develop an accurate grid-based lidar pointcloud upsampling method that preserves the geometry of the 3D environment. To this end, we go \textit{back to basics} and . Our analysis reveals that the upper and lower parts of the lidar pointcloud exhibit different point distributions. 2D convolutional networks (CNNs) which are trained in an end-to-end fashion without regard to the scene's geometry fail to account for these spatial discrepancies and tend to produce a point distribution that is somewhat close to the mean of these 2 distributions (see Figure~\ref{fig:teaser}).
